Using Voice and Biofeedback to Predict User Engagement during Product Feedback Interviews

Capturing users' engagement is crucial for gathering feedback about the features of a software product. In a market-driven context, current approaches to collect and analyze users' feedback are based on techniques leveraging information extracted from product reviews and social media. These approaches are hardly applicable in bespoke software development, or in contexts in which one needs to gather information from specific users. In such cases, companies need to resort to face-to-face interviews to get feedback on their products. In this paper, we propose to utilize biometric data, in terms of physiological and voice features, to complement interviews with information about the engagement of the user on the discussed product-relevant topics. We evaluate our approach by interviewing users while gathering their physiological data (i.e., biofeedback) using an Empatica E4 wristband, and capturing their voice through the default audio-recorder of a common laptop. Our results show that we can predict users' engagement by training supervised machine learning algorithms on biometric data (F1=0.72), and that voice features alone are sufficiently effective (F1=0.71). Our work contributes with one the first studies in requirements engineering in which biometrics are used to identify emotions. This is also the first study in software engineering that considers voice analysis. The usage of voice features could be particularly helpful for emotion-aware requirements elicitation in remote communication, either performed by human analysts or voice-based chatbots, and can also be exploited to support the analysis of meetings in software engineering research.

==> tables/table-confusion-biofeedback.tex <==
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllllll}
\multicolumn{9}{c}{\textit{\textbf{Arousal (Random Forest)}}} \\ \hline
\multicolumn{4}{c}{\textbf{Confusion matrix}} &  &  & \multicolumn{3}{c}{\textbf{Performance}} \\
 &  & \multicolumn{2}{l}{\textit{Predicted Label}} &  & \textit{Label} & \textit{Precision} & \textit{Recall} & \textit{F1} \\
\textit{} &  & Low & High &  & Low  & 0.71 & 0.81 & 0.76\\
\multirow{2}{*}{\textit{Gold Label}} & Low & 60 & 14 &  & High & 0.70 & 0.58 & 0.63 \\
 & High & 24 & 33 &  & macroAvg & 0.71 & 0.69 & 0.70 \\ \hline
\multicolumn{9}{c}{\textit{\textbf{Valence (SVM)}}} \\ \hline
\multicolumn{4}{c}{\textbf{Confusion matrix}} &  &  & \multicolumn{3}{c}{\textbf{Performance}} \\
 &  & \multicolumn{2}{l}{\textit{Predicted Label}} &  & \textit{Label} & \textit{Precision} & \textit{Recall} & \textit{F1} \\
\textit{} &  & Negative & Positive &  & Negative & 0.46 & 0.48 & 0.47 \\
\multirow{2}{*}{\textit{Gold Label}} & Negative & 13  & 14 &  & Positive & 0.86 & 0.86 & 0.86 \\
 & Positive & 15  & 89 &  & macroAvg & 0.66 & 0.67 & 0.67 
\end{tabular}%
}
\caption{Confusion matrices and performance by class for the best train-test round of the best algorithms, using biofeedback features, for Arousal (SVM) and Valence (Random Forest).}
\label{tab:confusionmatrixbiofeedback}
\end{table*}

%Best RNN Arousal
% {'results': {'0': {'precision': 0.7142857142857143, 'recall': 0.8108108108108109, 'f1-score': 0.759493670886076, 'support': 74}, '1': {'precision': 0.7021276595744681, 'recall': 0.5789473684210527, 'f1-score': 0.6346153846153846, 'support': 57}, 'accuracy': 0.7099236641221374, 'macro avg': {'precision': 0.7082066869300911, 'recall': 0.6948790896159318, 'f1-score': 0.6970545277507303, 'support': 131}, 'weighted avg': {'precision': 0.708995568342653, 'recall': 0.7099236641221374, 'f1-score': 0.7051573173179125, 'support': 131}}, 'confusion': Predicted   0   1  All
% Actual                
% 0          60  14   74
% 1          24  33   57
% All        84  47  131}

%BEST SVM Valence
% {'results': {'0': {'precision': 0.4642857142857143, 'recall': 0.48148148148148145, 'f1-score': 0.4727272727272727, 'support': 27}, '1': {'precision': 0.8640776699029126, 'recall': 0.8557692307692307, 'f1-score': 0.8599033816425121, 'support': 104}, 'accuracy': 0.7786259541984732, 'macro avg': {'precision': 0.6641816920943134, 'recall': 0.6686253561253561, 'f1-score': 0.6663153271848924, 'support': 131}, 'weighted avg': {'precision': 0.7816778011879176, 'recall': 0.7786259541984732, 'f1-score': 0.7801037256065467, 'support': 131}}, 'confusion': Predicted   0    1  All
% Actual                 
% 0          13   14   27
% 1          15   89  104
% All        28  103  131}



==> tables/table-confusion-combined.tex <==
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllllll}
\multicolumn{9}{c}{\textit{\textbf{Arousal (SVM)}}} \\ \hline
\multicolumn{4}{c}{\textbf{Confusion matrix}} &  &  & \multicolumn{3}{c}{\textbf{Performance}} \\
 &  & \multicolumn{2}{l}{\textit{Predicted Label}} &  & \textit{Label} & \textit{Precision} & \textit{Recall} & \textit{F1} \\
\textit{} &  & Low & High &  & Low & 0.78 & 0.84 & 0.81 \\
\multirow{2}{*}{\textit{Gold Label}} & Low & 62 & 12 &  & High & 0.76 &  0.68 & 0.72 \\
 & High & 18 & 39 &  & macroAvg & 0.77 & 0.76 & 0.76 \\ \hline
\multicolumn{9}{c}{\textit{\textbf{Valence (KNN)}}} \\ \hline
\multicolumn{4}{c}{\textbf{Confusion matrix}} &  &  & \multicolumn{3}{c}{\textbf{Performance}} \\
 &  & \multicolumn{2}{l}{\textit{Predicted Label}} &  & \textit{Label} & \textit{Precision} & \textit{Recall} & \textit{F1} \\
\textit{} &  & Negative & Positive &  & Negative & 0.79 & 0.41 & 0.54 \\
\multirow{2}{*}{\textit{Gold Label}} & Negative & 11 &  16 &  & Positive & 0.86 & 0.97 & 0.91 \\
 & Positive & 3 & 101 & & macroAvg & 0.82 & 0.70 & 0.72
\end{tabular}%
}
\caption{Confusion matrices and performance by class for the best train-test round of the best algorithms, using biofeedback features, for Arousal (SVM) and Valence (KNN).}
\label{tab:confusionmatrixcombine}
\end{table*}

%Best SVM Arousal
% {'results': {'0': {'precision': 0.775, 'recall': 0.8378378378378378, 'f1-score': 0.8051948051948051, 'support': 74}, '1': {'precision': 0.7647058823529411, 'recall': 0.6842105263157895, 'f1-score': 0.7222222222222222, 'support': 57}, 'accuracy': 0.7709923664122137, 'macro avg': {'precision': 0.7698529411764705, 'recall': 0.7610241820768137, 'f1-score': 0.7637085137085137, 'support': 131}, 'weighted avg': {'precision': 0.7705208801077683, 'recall': 0.7709923664122137, 'f1-score': 0.7690922309242919, 'support': 131}}, 'confusion': Predicted   0   1  All
% Actual                
% 0          62  12   74
% 1          18  39   57
% All        80  51  131}

%Best KNN Valence
% {'results': {'0': {'precision': 0.7857142857142857, 'recall': 0.4074074074074074, 'f1-score': 0.5365853658536585, 'support': 27}, '1': {'precision': 0.8632478632478633, 'recall': 0.9711538461538461, 'f1-score': 0.9140271493212669, 'support': 104}, 'accuracy': 0.8549618320610687, 'macro avg': {'precision': 0.8244810744810744, 'recall': 0.6892806267806267, 'f1-score': 0.7253062575874627, 'support': 131}, 'weighted avg': {'precision': 0.8472676602447595, 'recall': 0.8549618320610687, 'f1-score': 0.8362338046371034, 'support': 131}}, 'confusion': Predicted   0    1  All
% Actual                 
% 0          11   16   27
% 1           3  101  104
% All        14  117  131}

==> tables/table-confusion-voice.tex <==
\begin{table*}[h!]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{lllllllll}
\multicolumn{9}{c}{\textit{\textbf{Arousal (MLP)}}} \\ \hline
\multicolumn{4}{c}{\textbf{Confusion matrix}} &  &  & \multicolumn{3}{c}{\textbf{Performance}} \\
 &  & \multicolumn{2}{l}{\textit{Predicted Label}} &  & \textit{Label} & \textit{Precision} & \textit{Recall} & \textit{F1} \\
\textit{} &  & Low & High &  & Low & 0.73 & 0.80 & 0.76 \\
\multirow{2}{*}{\textit{Gold Label}} & Low & 59 & 15 &  & High & 0.7 & 0.61 & 0.65 \\
 & High & 22 & 35 &  & macroAvg & 0.71 & 0.71 & 0.71 \\ \hline
\multicolumn{9}{c}{\textit{\textbf{Valence (MLP)}}} \\ \hline
\multicolumn{4}{c}{\textbf{Confusion matrix}} &  &  & \multicolumn{3}{c}{\textbf{Performance}} \\
 &  & \multicolumn{2}{l}{\textit{Predicted Label}} &  & \textit{Label} & \textit{Precision} & \textit{Recall} & \textit{F1} \\
\textit{} &  & Negative & Positive &  & Negative & 0.58 & 0.52 & 0.55 \\
\multirow{2}{*}{\textit{Gold Label}} & Negative & 14 & 13 &  & Positive & 0.89 & 0.90 & 0.89 \\
 & Positive & 10 & 94 &  & macroAvg & 0.73 & 0.71 & 0.72
\end{tabular}%
}
\caption{Confusion matrices and performance by class for the best train-test round of the best algorithm (Multi-layer Perceptron), using biofeedback features, for Arousal and Valence.}
\label{tab:confusionmatrixvoice}
\end{table*}


%best MLP run arousal
% {'results': {'0': {'precision': 0.7283950617283951, 'recall': 0.7972972972972973, 'f1-score': 0.7612903225806451, 'support': 74}, '1': {'precision': 0.7, 'recall': 0.6140350877192983, 'f1-score': 0.6542056074766356, 'support': 57}, 'accuracy': 0.7175572519083969, 'macro avg': {'precision': 0.7141975308641975, 'recall': 0.7056661925082978, 'f1-score': 0.7077479650286403, 'support': 131}, 'weighted avg': {'precision': 0.7160399585335971, 'recall': 0.7175572519083969, 'f1-score': 0.7146962099018013, 'support': 131}}, 'confusion': Predicted   0   1  All
% Actual                
% 0          59  15   74
% 1          22  35   57
% All        81  50  131}

%best MLP run valence
% {'results': {'0': {'precision': 0.5833333333333334, 'recall': 0.5185185185185185, 'f1-score': 0.5490196078431373, 'support': 27}, '1': {'precision': 0.8785046728971962, 'recall': 0.9038461538461539, 'f1-score': 0.8909952606635071, 'support': 104}, 'accuracy': 0.8244274809160306, 'macro avg': {'precision': 0.7309190031152648, 'recall': 0.7111823361823362, 'f1-score': 0.7200074342533223, 'support': 131}, 'weighted avg': {'precision': 0.8176678319183848, 'recall': 0.8244274809160306, 'f1-score': 0.820511729166179, 'support': 131}}, 'confusion': Predicted   0    1  All
% Actual                 
% 0          14   13   27
% 1          10   94  104
% All        24  107  131}

==> tables/table-smote-biofeedback.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lllllll}
\hline
\multicolumn{1}{|l|}{}          & \multicolumn{3}{c|}{\textit{Valence}}                                          & \multicolumn{3}{c|}{\textit{Arousal}}                                          \\ \hline
\multicolumn{1}{|l|}{algorithm} & \multicolumn{1}{l|}{Prec} & \multicolumn{1}{l|}{Rec} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{Prec} & \multicolumn{1}{l|}{Rec} & \multicolumn{1}{l|}{F1} \\ \hline

SVM	&0.891	&0.940	&0.912	&0.913	&0.917	&0.914 \\
MLP	&0.998	&0.998	&0.998	&\textbf{0.980}	&\textbf{0.981}	&\textbf{0.981} \\
KNN	&\textbf{1.000}	&\textbf{1.000}	&\textbf{1.000}	&0.787	&0.790	&0.786 \\
Dtree	&0.952	&0.977	&0.962	&0.977	&0.979	&0.977 \\
NB	&0.548	&0.549	&0.506	&0.582	&0.522	&0.386 \\
RNN	&0.978	&0.973	&0.975	&0.975	&0.974	&0.974 
\end{tabular}
\caption{Comparison of the performance of the different supervised learning algorithms using biofeedback features and SMOTE.}
\label{tab:performancecomparisonsmote}
\end{table}

==> tables/table-smote-combined.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lllllll}
\hline
\multicolumn{1}{|l|}{}          & \multicolumn{3}{c|}{\textit{Valence}}                                          & \multicolumn{3}{c|}{\textit{Arousal}}                                          \\ \hline
\multicolumn{1}{|l|}{algorithm} & \multicolumn{1}{l|}{Prec} & \multicolumn{1}{l|}{Rec} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{Prec} & \multicolumn{1}{l|}{Rec} & \multicolumn{1}{l|}{F1} \\ \hline
SVM	&0.993	&0.998	&0.995	&0.976	&0.973	&0.974 \\
MLP	&0.998	&1.000	&0.999	&0.983	&0.983	&0.983 \\
KNN	&\textbf{1.000}	&\textbf{1.000}	&\textbf{1.000}	&\textbf{1.000}	&\textbf{1.000}	&\textbf{1.000} \\
Dtree	&0.908	&0.962	&0.930	&0.948	&0.950	&0.946 \\
NB	&0.607	&0.644	&0.610	&0.637	&0.637	&0.627 \\
RNN	&0.973	&0.964	&0.968	&0.974	&0.975	&0.974            
\end{tabular}
\caption{Comparison of the performance of the different supervised learning algorithms using combined features and SMOTE.
}
\label{tab:performancecomparisoncombinesmote}
\end{table}

==> tables/table-smote-voice.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{lllllll}
\hline
\multicolumn{1}{|l|}{}          & \multicolumn{3}{c|}{\textit{Valence}}                                          & \multicolumn{3}{c|}{\textit{Arousal}}                                          \\ \hline
\multicolumn{1}{|l|}{algorithm} & \multicolumn{1}{l|}{Prec} & \multicolumn{1}{l|}{Rec} & \multicolumn{1}{l|}{F1} & \multicolumn{1}{l|}{Prec} & \multicolumn{1}{l|}{Rec} & \multicolumn{1}{l|}{F1} \\ \hline
SVM	&0.959	&0.978	&0.968	&0.926	&0.926	&0.926 \\
MLP	&\textbf{0.967}	&\textbf{0.979}	&\textbf{0.972}	&\textbf{0.978}	&\textbf{0.974}	&\textbf{0.975} \\
KNN	&\textbf{0.967}	&\textbf{0.979}	&\textbf{0.973}	&0.957	&0.959	&0.957 \\
Dtree	&0.858	&0.930	&0.881	&0.953	&0.947	&0.949 \\
NB	&0.584	&0.621	&0.576	&0.625	&0.626	&0.622 \\
RNN	&0.940	&0.948	&0.943	&0.957	&0.955	&0.956          
\end{tabular}
\caption{Comparison of the performance of the different supervised learning algorithms using voice-related features and SMOTE.}
\label{tab:performancecomparisonvoicesmote}
\end{table}


